A scalable solver for a stochastic, hybrid cellular automaton model of personalized breast cancer therapy

Mathematical modeling and simulation is a promising approach to personalized cancer medicine. Yet, the complexity, heterogeneity and multi-scale nature of cancer pose significant computational challenges. Coupling discrete cell-based models with continuous models using hybrid cellular automata is a powerful approach for mimicking biological complexity and describing the dynamical exchange of information across different scales. However, when clinically relevant cancer portions are taken into account, such models become computationally very expensive. While efficient parallelization techniques for continuous models exist, their coupling with discrete models, particularly cellular automata, necessitates more elaborate solutions. Building upon FEniCS, a popular and powerful scientific computing platform for solving partial differential equations, we developed parallel algorithms to link stochastic cellular automata with differential equations ( https://bitbucket.org/HTasken/cansim ). The algorithms minimize the communication between processes that share cellular automata neighborhood values while also allowing for reproducibility during stochastic updates. We demonstrated the potential of our solution on a complex hybrid cellular automaton model of breast cancer treated with combination chemotherapy. On a single-core processor, we obtained nearly linear scaling with an increasing problem size, whereas weak parallel scaling showed moderate growth in solving time relative to increase in problem size. Finally we applied the algorithm to a problem that is 500 times larger than previous work, allowing us to run personalized therapy simulations based on heterogeneous cell density and tumor perfusion conditions estimated from magnetic resonance imaging data on an unprecedented scale.

==> cut.tex <==
\subsection{Scalability and efficiency tests}
\label{sec:scalability_tests}

\subsection{Solver setups}

For each PDE solver, report and justify: Solver, Preconditioner and tolerances

Since the aim is to solve large scale problems, you focus on iterative methods rather than direct methods. Iterative methods are expected to scale well to large problem sizes and across many CPUs.

Chemotherapy:
\begin{itemize}
    \item Krylov solver: CG (system is symmetric and positive definite).
    \item Preconditioner: algebraic multigrid (BoomerAMG) (why: algebaric multigrid is well suited for this problem (find references). HypreAMG is a well established library with a robust implementation.
          Show BoomerAMG special settings (e.g. ext+i) and justify them.
    \item Tolerances: relative and absolute tolerance: $10^{-8}$.
\end{itemize}


Oxygen:
\begin{itemize}
    \item Non-linear solver: Newton
    \item Krylov solver: CG (system is symmetric and positive definite).
    \item Preconditioner: Jacobi (for small timesteps and $D_k$ values, the linear system (23) is close to a discrete identity operator (mass matrix)). 
    \item Tolerances: relative and absolute tolerance: ??
\end{itemize}


Coupled PDE:
\begin{itemize}
    \item Non-linear solver: Newton
    \item Krylov solver: GMRES (system is not-symmetric).
    \item Preconditioner: Jacobi (for small timesteps and $D_k$ values, the linear system (23) is close to a discrete identity operator (mass matrix). 
    \item Tolerances: relative and absolute tolerance: ??
\end{itemize}


\subsection{Overall timing}
For this section, we will be showing the timing of a $100 \times 100$ grid simulation, equivalent of a physical size of $\SI{1}{\mm^2}$ with a typical cell density of 0.4 and vessel density of 0.12. The average intra- and inter-update timing of the solver was carried out on a single core CPU.
As shown in \cref{fig:intra_timing,fig:inter_timing}, the total timing are broken down by processes (\cref{fig:intra_timing_a,fig:inter_timing_a}) and by model modules (\cref{fig:intra_timing_b,fig:inter_timing_b}).  \hfill\\

Within $\Delta t_{\text{update}} = \SI{30}{\min}$, a smaller $dt = \SI{1}{\min}$ was used for the solving of PDEs. 
The assembly of the discrete PDE operators takes the majority of the time, specifically the time-dependent assembly of the non-linear PDEs, followed by solving and other cost such as initialization. 
ODE solving time is minimal as it is vectorized and solved for all points in the grid. 
The breakdown by modules shed some insights on the cost of assembly:
the solution of both VAC and Oxygen modules are obtained by solving non-linear PDEs, and the system is re-assembled for each $dt$. Due to the nature of the non-linearity, it cannot be pre-assembled to save time.
Time spent on chemotherapy module comes second as there are three types of chemotherapies to be solved separately. 
Initialization includes mesh initialization as well as function initialization for each module. This is done only once at the beginning of the whole simulation.

Overall we found similar cost distribution comparing intra- and inter-update, implying communication during discrete updates were efficient.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main/component1}
        \caption{Intra-update timing of the solver grouped by processes}
        \label{fig:intra_timing_a}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main/component2}
        \caption{Intra-update timing of the solver grouped by modules of the model}  
        \label{fig:intra_timing_b}
    \end{subfigure}
    \caption{Intra-update timing of the model with $\Delta t = \SI{1}{min}$ solved for $t=\SI{30}{min}$.}
    \label{fig:intra_timing}
\end{figure} 

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main/component1_inter}
        \caption{Average inter-update timing of the solver grouped by processes}
        \label{fig:inter_timing_a}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/main/component2_inter}
        \caption{Average inter-update timing of the solver grouped by modules of the model}
        \label{fig:inter_timing_b}
    \end{subfigure}
    \caption{Average inter-update timing of the model with $\Delta t = \SI{30}{min}$ solved over $t=\SI{120}{min}$.}
    \label{fig:inter_timing}
\end{figure}
  
\subsubsection{Spatial scalability}
Given the distribution of time spent on each modules, we are also interested in how well the model scales given increasing problem size on a a single core. 
This allows us to establish the scalability of the algorithm without interference of overhead cost from MPI communications. It is also beneficial for establishing the maximum size of a problem that can be solved until memory size is a concern.

In \cref{fig:spatial}, we achieved an almost linear scaling for the PDE components in all three modules. The assembly time in VAC takes slightly longer on larger problems due to the cost of constructing preconditioner for the iterative solver. 
As the memory in our single core setup is limited to an usable amount of 4GB, we were unable to run problems containing grid points of number larger than $10^5$. For this reason, we chose an iterative solver over direct solver such as superLU and MUMPS.

Main result (example - check):
\begin{itemize}
    \item The assembly scales nearly perfectly in serial.
    \item The sovler scales ???
\end{itemize}



\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/main/space}
    \caption{Illustration of spatial scaling of all PDEs within $\Delta t = \SI{30}{min} $ of simulations with number of grid points up to $10^5$. Assembly and Solving times were shown in solid and dotted line in all panels}
    \label{fig:spatial}
\end{figure}

\subsubsection{Parallel scalability}

We investigate the scalability of solving the PDE equations involved the mathematical model, specifically the weak scaling. Weak scaling is when problem size (workload) assigned to each processing element stays constant and additional elements are used to solve a larger total problem on more CPU cores. In specific, the degrees of freedoms (DOFs) assigned to each processor are kept the same while additional processors are used to solve problem on larger meshes with more DOFs. In the case of weak scaling, perfect scaling is achieved if the run time stays constant while the workload is increased in direct proportion to the number of processors.

We are interested in knowing the weak scaling of assembly and solving time corresponding to each PDE solver. Weak Scaling Efficiency (WSE), defined as
\begin{align}
    WSE = \frac{t_N}{t_1} 100\% ,
\end{align}
is calculated for assembly and solving time separately. $t_1$ and $t_N$ are the time it take to complete the task using 1 and $N$ processors respectively. 

Abel, the high performance computing facility at UiO hosted at USIT, composes all dual Intel E5-2670 (Sandy Bridge) based running at 2.6 GHz, Each node yields 16 physical compute cores with 64 GiBytes of Samsung DDR3 memory operating at 1600 MHz, giving 4 GiB memory per physical core.

FEniCS version 2018.1.0 with PETSc was built with Intel compiler.
The scalability tests of PDEs were out on a interactive login shell with two nodes, 32 physical cores in total, with exclusive access to minimize communication overhead. Results are shown below.

For the sake of comparison, the end time of all temporal updates of PDEs in the model was set to $t = 30 \text{ min} $, cell and vessel configurations were initialized randomly and the densities of cells and vessels were set to $0.4$ and $0.1197$ to reflect scenarios of real patient simulation.

\subsubsection{Poisson equation scaling}
We will first establish the scalability on a simplified problem, namely the Poisson equation by finding the appropriate preconditioner and solver setup. 

The 2D Poisson problem is governed by
\begin{align}
    - \nabla^2 u &= f \quad \text{ in } \Omega\\
    \intertext{with}
    \Omega &= [0,1] \times [0,1] \notag\\
    \Gamma_{D} &= \{(0, y) \cup (1, y) \subset \partial \Omega\} \notag\\
    \Gamma_{N} &= \{(x, 0) \cup (x, 1) \subset \partial \Omega\} \notag\\
    g &= \sin(5x) \notag\\
    f &= 10\exp(-((x - 0.5)^2 + (y - 0.5)^2) / 0.02)
\end{align}

The following options were used for the linear PETSc Krylov solver:
\begin{verbatim}
PETScOptions.set("ksp_max_it", 5000)
PETScOptions.set("ksp_rtol", 1e-8)
PETScOptions.set("ksp_atol",1e-8)
PETScOptions.set("ksp_view")
PETScOptions.set("ksp_converged_reason")
PETScOptions.set("ksp_monitor_true_residual")
PETScOptions.set("ksp_type", "cg")
PETScOptions.set("pc_type", "hypre")
PETScOptions.set("pc_hypre_type", "boomeramg")
PETScOptions.set("pc_hypre_bommeramg_strong_threshold", 0.5)
PETScOptions.set("pc_hypre_boomeramg_interp_type","ext+i")
\end{verbatim}

\begin{table}
\begin{center}
    \input{tables/main/poisson_timing}
\end{center}
\caption{Poisson timing}
\label{tab:poisson_timing}
\caption{Timing of Poisson solve. Results shown are the minimum of 5 repeated runs. }
\end{table}

we did not achieve perfect scaling of the Poisson problem with the current setup, possibly due to too few numbers of DOFs. However we were limited to $<10^7$ of DOFs before the memory usage becomes a problem.

\subsubsection{Chemotherapy equation scaling}
The temporal update of chemotherapy was investigated (\cref{tab:chemo_timing}). The temporal discretization is done using Crank-Nicolson scheme. By inspecting the PDE \cref{eq:chemo}, the left hand side is constant in $G$. We were therefore able to reduce the overall update time by pre-assembly of the matrix. The same options for the linear solver were used. 



\begin{table}
\begin{center}
    \input{tables/main/chemo_timing}
\end{center}
\caption{Timing of temporal chemo update ($t$ = 30 min). $dt$ was kept constant during the update and the results shown are the minimum of 5 repeated runs of the updates with random initialization of cell and vessel configurations. Intracvascular concentration was kept constant during the testing}
\label{tab:chemo_timing}
\end{table}

\subsubsection{Oxygen equation scaling}
The temporal discretization is treated the same as chemotherapy PDE using Crank-Nicolson scheme.  In \cref{eq:oxygen}, it has a non-linear forcing term. We took the automatic approach where FEniCS attacks the nonlinear variational problem with a Newton scheme.
The newton solver was used to iterate between updates and Krylov solver was used to solve the linear variational problem to provide the guess of each iteration. We did not cache the assembled left hand side (the Jacobian) during each update, resulting in almost double the amount of assembly time  \cref{tab:oxygen_timnig}


\begin{table}
\begin{center}
    \input{tables/main/oxygen_timing}
\end{center}
\caption{Timing of temporal oxygen update ($t$ = 30 min). $dt$ was kept constant during the update and the results shown are the minimum time of 5 repeated runs of the updates with random initialization of cell and vessel configurations.}
\label{tab:oxygen_timnig}
\end{table}

\subsubsection{V-A-C coupled equation scaling}
As before, the temporal discretization is treated the same as chemotherapy PDE using Crank-Nicolson scheme.  The forcing term is a nonlinear function of the variable VAC. We use FEniCS to solve the nonlinear variational problem directly. Newton solver was used to iterate between updates and Krylov solver was used to solve the linear variational problem to provide the guess of each iteration. 

\begin{table}[h]
\begin{center}
    \input{tables/main/vac_timing}
\end{center}
\caption{Timing of temporal VAC update ($t$ = 30 min). $dt$ was kept constant during the update and the results shown are the minimum of 5 repeated runs of the updates with random initialization of cell and vessel configurations.}
\label{tab:VAC_timnig}
\end{table}

\begin{figure}
    \centering
    \includegraphics[draft=false,width=\textwidth]{figures/main/parallel}
    \caption{Illustration of Weak Scaling Efficiency of all PDEs}
    \label{fig:WSE}
\end{figure}


Weak scaling results are summarized in \cref{fig:WSE}, using the PETSc GMRES solver with AMG (algebraic multigrid) preconditioner for the nonlinear equations, and PETSc CG solver with Hypre BoomerAMG for the linear ones. 
The matrix assembly phase scales well. The modest growth in the time for the preconditioned Krylov solver can be attributed in part to a modest increase (roughly 10\%) in the iteration count over the 32 fold increase in problem size. 
We have put limited effort into tuning the multigrid preconditioners for this problem as it falls outside the scope of work. 
Some improvements may be possible through tuning of the preconditioners. 

%\section{Application}
\label{sec:application}


==> tables/main/poisson_timing.tex <==
\begin{tabular}{|p{0.5cm}||p{1.5cm}|c|p{1.3cm}|p{1.5cm}|c|c|c|c|}
\toprule
    & Number of Krylov iterations & Number of Processes & Total dofs & Average dof per process & Assembly & Assembly WSE & Solve  & Solve WSE \\ \midrule
1   & 9                           & 1                   & 159600     & 159600                  & 0.81509  & 1            & 1.0887 & 1         \\
8   & 12                          & 8                   & 1280292    & 160036                  & 0.78809  & 0.96687      & 1.6816 & 1.5446    \\
16  & 12                          & 16                  & 2558400    & 159900                  & 0.97599  & 1.1974       & 2.373  & 2.1797    \\
24  & 11                          & 24                  & 3839640    & 159985                  & 1.0057   & 1.2339       & 2.7522 & 2.528     \\
32  & 12                          & 32                  & 5118906    & 159965                  & 1.1672   & 1.432        & 2.9707 & 2.7287    \\
40  & 13                          & 40                  & 6398370    & 159959                  & 1.2198   & 1.4965       & 3.1726 & 2.9141    \\
80  & 13                          & 80                  & 12798506   & 159981                  & 1.3156   & 1.6141       & 3.1875 & 2.9278    \\
120 & 13                          & 120                 & 19197542   & 159979                  & 1.3099   & 1.6071       & 4.0632 & 3.7322    \\ \bottomrule
\end{tabular}

==> tables/main/vac_timing.tex <==
\begin{tabular}{|p{0.5cm}||p{1.5cm}|c|p{1.3cm}|p{1.5cm}|c|c|c|c|}
\hline
& Total dofs & Number of Processes & Average dof per process & Assembly & Assembly WSE & Solve & Solve WSE \\
\hline\hline
1 & 159197 & 1 & 159197 & 450.13 & 1 & 675.41 & 1 \\
\hline
2 & 321485 & 2 & 160742 & 568.35 & 1.1058 & 774.65 & 1.1469 \\
\hline
4 & 638397 & 4 & 159599 & 593.76 & 1.0793 & 845.83 & 1.2523 \\
\hline
8 & 1279157 & 8 & 159894 & 630.66 & 1.1464 & 893.31 & 1.4167 \\
\hline
16 & 2556797 & 16 & 159799 & 981.5 & 2.0622 & 1447.2 & 2.3349 \\
\hline
\end{tabular}


1 & 1 & 477591 & 4.7759e+05 & 5.7243 & 1 & 7.3177 & 1 \\
\hline
8 & 8 & 3837471 & 4.7086e+05 & 6.2225 & 1.087 & 21.9 & 2.9927 \\
\hline
16 & 16 & 7670391 & 4.6778e+05 & 6.7417 & 1.1777 & 28.668 & 3.9176 \\
\hline
24 & 24 & 11513031 & 4.5989e+05 & 6.9127 & 1.2076 & 34.383 & 4.6986 \\
\hline
32 & 32 & 15363495 & 4.504e+05 & 7.4316 & 1.2983 & 35.468 & 4.8469 \\
\hline
40 & 40 & 19217871 & 4.2815e+05 & 7.5204 & 1.3138 & 38.831 & 5.3064 \\
\hline
80 & 80 & 38427711 & 4.6716e+05 & 7.844 & 1.3703 & 44.281 & 6.0512 \\
